Relation-Aware Language-Graph Transformer for Question Answering

Question Answering (QA) is a task that entails reasoning over natural language contexts, and many relevant works augment language models (LMs) with graph neural networks (GNNs) to encode the Knowledge Graph (KG) information. However, most existing GNN-based modules for QA do not take advantage of rich relational information of KGs and depend on limited information interaction between the LM and the KG. To address these issues, we propose Question Answering Transformer (QAT), which is designed to jointly reason over language and graphs with respect to entity relations in a unified manner. Specifically, QAT constructs Meta-Path tokens, which learn relation-centric embeddings based on diverse structural and semantic relations. Then, our Relation-Aware Self-Attention module comprehensively integrates different modalities via the Cross-Modal Relative Position Bias, which guides information exchange between relevant entites of different modalities. We validate the effectiveness of QAT on commonsense question answering datasets like CommonsenseQA and OpenBookQA, and on a medical question answering dataset, MedQA-USMLE. On all the datasets, our method achieves state-of-the-art performance. Our code is available at http://github.com/mlvlab/QAT.

==> C_additional_analysis/obqa_leaderboard.tex <==
\input{Tables/obqa_leaderboard.tex}

==> C_additional_analysis/qualitative_analysis.tex <==
\paragraph{Qualitative analyses.}
\input{Figures/tex/suppl_matching}
In Figure~\ref{sup_fig:qual} and~\ref{sup_fig:quali_matching}, we provide additional qualitative examples for what we have shown in Figure 3 and 4 of the main paper.
Similar to the main paper, the RASA maps for the correct answer choice generally show smooth values across KG and LM, whereas wrong choices tend to have weaker cross-modal attention.
Furthermore, it is also noteworthy that the Meta-Path token set size (\ie, the KG portion) is very diversified in most examples, indicating a greater KG expressivity for self-attention.

==> Figures/tex/suppl_choice.tex <==
\begin{figure*}[t!]
\centering
% \subfigure[]{
% \includegraphics[width=1\columnwidth]{Figures/img/suppl_choice_1.pdf}
% }
\subfigure[]{
\includegraphics[width=1\columnwidth]{Figures/img/suppl_choice_2.pdf}
}
\subfigure[]{
\includegraphics[width=1\columnwidth]{Figures/img/suppl_choice_3.pdf}
}
% \subfigure[]{
% \includegraphics[width=1\columnwidth]{Figures/img/suppl_choice_4.pdf}
% }
\caption{ \textbf{Additional examples of QAT attention maps by each answer choice.}}
\label{sup_fig:qual}
\end{figure*}

==> Figures/tex/suppl_matching.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=1\columnwidth]{Figures/img/suppl_matching.pdf}
\end{center}
% \vspace{5mm}
\caption{\textbf{Additional example of the effect of Cross-Modal Relative Position Bias.}}
\label{sup_fig:quali_matching}
\end{figure}


==> Tables/analysis_edgeaug.tex <==
\begin{table}[h!]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \resizebox{0.8\columnwidth}{!}{
    \begin{tabular}{c c c}
        \toprule
        \textbf{top-$k$ edges}  & \textbf{IHdev-Acc}(\%) & \textbf{IHtest-Acc}(\%) \\
        \midrule
        \midrule
        1     &      &       \\
        3     &  79.0 (±0.6)    &  75.3 (± 0.7)     \\
        10     &      &       \\
        30     &      &       \\
        \bottomrule
    \end{tabular}
    }
    \caption{Sensitivity analysis on the top-$k$ edge augmentation on CommonsenseQA.}
    \label{tab:edgeaug}
\end{table}


==> Tables/analysis_gnn_ours2.tex <==
\begin{table}[h!]
    \centering
    \setlength{\tabcolsep}{4.0pt}
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{l c c}
        \toprule
        \textbf{Dataset}         & \textbf{GNN Encoder} & \textbf{Meta-Path Tokens} \\
        \midrule
        \midrule
        CommonsenseQA                      &  73.9 ($\pm$ 0.2)  &  \textbf{75.3 ($\pm$ 0.7)} \\
        OpenBookQA                         &  69.6 ($\pm$ 0.9)  &  \textbf{70.9 ($\pm$ 0.8)} \\
        OpenBookQA (AristoRoBERTa)         &  86.3 ($\pm$ 0.8)  &  \textbf{86.9 ($\pm$ 0.2)} \\
        \bottomrule
    \end{tabular}
    }
    \caption{GNN encoder and Meta-Path Token Comparison.}
    \label{tab:gnn_ours2}
\end{table}


==> Tables/csqa_leaderboard.tex <==
\begin{table}[ht!]
    \centering
    \setlength{\tabcolsep}{3.0pt}
    \begin{tabular}{l c}
        \toprule
        \textbf{Methods} & \textbf{Acc.}\\
        \midrule
        \midrule
        RoBERTa & 72.1 \\
        ALBERT & 76.5 \\
        \midrule
        RoBERTa + FreeLB & 73.1 \\
        RoBERTa + HyKAS & 73.2 \\
        RoBERTa + KE & 73.3 \\
        RoBERTa + KEDGN & 74.4 \\
        XLNet + GraphReason & 75.3 \\
        RoBERTa + MHGRN & 75.4 \\
        ALBERT + PG & 75.6 \\
        RoBERTa + QA-GNN & 76.1 \\
        RoBERTa + JointLK & 76.6 \\
        RoBERTa + GSC & 76.4 \\
        RoBERTa + QAT \textbf{(ours)} & 0.0\\
        \bottomrule
    \end{tabular}
    \caption{Performance comparison on \textit{CommonsenseQA} official leaderboard.}
    \label{tab:csqa_leaderboard}
\end{table}

% JointLK table 2

==> Tables/suppl_mptoken.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{c c c}
        \toprule
        \textbf{max $K$-hops }  & \textbf{IHdev-Acc}(\%) & \textbf{IHtest-Acc}(\%) \\
        \midrule
        \midrule
        1     &      &       \\
        2     & 79.5 (± 0.4)     &  75.4 (± 0.3)     \\
        3     &      &       \\
        \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Sensitivity analysis of the maximum hop used for Meta-Path tokens.}}
    \label{tab:mptoken}
\end{table}


==> algorithm.tex <==
\clearpage

\begin{algorithm}
\caption{Pseudocode} 
\textbf{Input:} Input tokens $\left\{\lmin\right\}$, graph $\graph$, nodefeat $\left\{\nodefeat_i\right\}$\\
\textbf{Output:} network parameter $\theta$

% \setstretch{1.3}
\begin{algorithmic}[1]
\State $\left\{\lmout_{cls}, \lmout_1, \dots, \lmout_N\right\} \leftarrow \mbox{LM}\left(\left\{\lmin_{cls}, \lmin_1, \dots, \lmin_N\right\} \right)$

\State $\graph^\prime \leftarrow \mbox{G-aug}\left(\graph\right)$
\For{$k=1,\dots, K$}
    \State $\pathset_k\left(\node_j, \node_i \right) \leftarrow \mbox{Extract}\left(\graph^\prime \right), \forall \node_j, \node_i \in \graph^\prime$
    \State $\kgout_{\paths_k(v_j, v_i)} \leftarrow \mbox{MLP}_{\theta_k}\left(\paths_k(v_j, v_i)\right)$
\EndFor
\For{$l=1, \dots L$}
    \State $\left\{\boldsymbol{o}_{cls}, \dots \right\} \leftarrow \mbox{Transformer}\left(\left\{\lmout_{cls}, \dots, \lmout_N, \kgout_\phi \right\} \right)$
\EndFor
\State $\tilde{\mathbf{o}} \leftarrow \mbox{MLP}\left(\mathbf{o}_{cls} \right) $

\end{algorithmic} 
\end{algorithm}

==> candidates.tex <==
\section{Title Candidates}
\begin{itemize}
    \item Graph Relation Transformer for Question Answering 
    \item Relation in Relation: Encoding the relation for Question Answering with Knowledge Graphs (RnR) ***
    \item Relational Transformer Network (ReTraNet)
    \item Relation Network Transformer (RENT)
    \item Relation is All You Need *
    \item Encoding Relation with Relation Encoding 
    \item Reasoning with Language Models and Graph Transformers for Question Answering
    \item Relational Reasoning with Graph Transformers for Knowledge-Aware Question Answering **  
    \item Relation-Aware Reasoning with (Interaction?) (Relation?) Graph Transformer for Question Answering
    \item QA-Transformer: Knowledge Graph Transformer for Question Answering
    \item QAT: Knowledge Graph Transformer for Question Answering ***
    \item KGT: Knowledge Graph Transformer for Question Answering **
    \item Relation Transformer for Question Answering with Knowledge Graphs
    \item Language-Interaction Transformer for Question Answering
    \item Language-Interaction Transformer for Question Answering with Relation Networks
    \item Encoding Interactions: Relation Transformer for Question Answering with Knowledge Graphs
    \item Relation-Aware Reasoning for Question Answering **
    \item Relation-Aware Transformer Networks for Question Answering ***
    \item Multimodal Relational Reasoning for Question Answering with Knowledge Graphs
    \item Multimodal Transformer for Knowledge-based Question Answering
    \item K-QAT
    \item KG-QAT
    \item QAGL Transformer
    \item Multimodal Question Answering Transformer
    \item Question Answering Transformer with Knowledge Graphs
    \item Multi-relational Transformer
    \item Encoding Relations with Graph-Language(text?) Transformer for Knowledge-based Question Answering
    \item \textbf{Token Relation-guided Transformer for Knowledge-based Question Answering}
    \item mQA Transformer
    \item Text-Graph Mixer
    \item TRTR : Token Relation-guided Transformer
    \item $\text{TR}^2$ : Token Relation-guided Transformer
    \item trTR
    \item Relation-to-Token
    \item Metapath-to-Token 
    \item Language-Graph Transformer
    \item RelT RelTr
    \item ReLaTe: \textbf{Re}lation-guided \textbf{La}nguage-Graph \textbf{T}ransform\textbf{e}r for Question Answering
    \item ReLaTR: \textbf{Re}lation-guided \textbf{La}nguage-Graph
    \item RELATR: Relation-guided Language-Graph Transformer for Question Answering
    \item QAT: Relation-aware Question Answering with Transformers for (Language and Graph?) %DETR따라하기..
    \item rLGT
    \item LaphTr
    \item LaGr
    
\end{itemize}
